Finite-Word Hyperlanguages

Formal languages are in the core of models of computation and their behavior. A rich family of models for many classes of languages have been widely studied. Hyperproperties lift conventional trace-based languages from a set of execution traces to a set of sets of executions. Hyperproperties have been shown to be a powerful formalism for expressing and reasoning about information-flow security policies and important properties of cyber-physical systems. Although there is an extensive body of work on formal-language representation of trace properties, we currently lack such a general characterization for hyperproperties. We introduce hyperlanguages over finite words and models for expressing them. Essentially, these models express multiple words by using assignments to quantified word variables. Relying on the standard models for regular languages, we propose hyperregular expressions and finite-word hyperautomata (NFH), for modeling the class of regular hyperlanguages. We demonstrate the ability of regular hyperlanguages to express hyperproperties for finite traces. We explore the closure properties and the complexity of the fundamental decision problems such as nonemptiness, universality, membership, and containment for various fragments of NFH.

==> HLTLtoNBH.tex <==
\subsection{HyperLTL to HyperABH}

{\em HyperLTL}~\cite{cfkmrs14} is a logic for expressing hyperproperties, based on the syntax of LTL.
While an LTL formula describes the behavior of a single trace, a hyperLTL formula describes the behavior of a set of traces, by using quantified {\em trace variables} over an LTL formula that uses these variables to describe the traces that are assigned to them. 
For example, the HyperLTL formula 
$$\g = \forall x. \exists y. \globally(a_x \Leftrightarrow a_y)$$
requires that for every trace $\pi$ in a set $S$ that satisfies $\g$ there exists a trace that agrees with $\pi$ on the positions that satisfy the atomic proposition $a$. 
For the full definition of HyperLTL, see~\cite{cfkmrs14}. 

\todo{We can move the syntax and semantics of HyperLTL to the appendix.}

%\subsection {HyperLTL~\cite{cfkmrs14}}


\stam{

Let $\AP$ be a set of atomic propositions. A {\em trace $t = t_0t_1\cdots$ over $AP$}  is an infinite word over $2^{\AP}$.

We assume that the reader is familiar with the syntax and semantics of LTL. The syntax of HyperLTL uses {\em trace variables} , and is defined by the following grammar.
%
\begin{align*}
\hspace{3cm}\psi & ::= \exists\pi.\psi \mid \forall\pi.\psi \mid \f\\
\f & ::= a_\pi \mid  \neg\f \mid  \f\vee\f \mid  \nextt\f \mid  \f\until\f
\end{align*}
%
where $a \in \AP$, $\pi$ is a trace variable from an infinite supply $\Pi$.
Intuitively, HyperLTL expresses LTL properties of sets of traces, where $\exists \pi$ means that the property is true for some trace in the set, and $\forall \pi$ means that the property is true for all traces in the set. 

Formally, the semantics of HyperLTL is as follows.
Let $T$ be a set of traces, let $\Pi$ be an (infinite) set of trace variables, and let $v:\Pi\rightarrow T$ be a partial function. We denote $v^i = \{v(\pi)^i \mid \pi\in \Pi\}$ the $i$-shift of all traces assigned by $v$ (i.e., the suffixes starting from position $i$)\todo{BB: I think this is what you meant.}.
We define a satisfaction relation $\models$ for an assignment $v:\Pi\rightarrow T$ and a HyperLTL formula $\f$, as follows.
%
\[
\begin{array}{l@{\hspace{2em}}c@{\hspace{2em}}l}
T\models _v \exists\pi.\psi & \text{iff} & \text{there exists} \ t \in T \ \text{such that} \ T\models_{v[\pi\mapsto t]\psi}\\
%
T\models _v \forall\pi.\psi & \text{iff} & \text{for every} \ t\in T \ \text{it holds that} \ T\models_{v[\pi\mapsto t]\psi}\\
T\models _v a_\pi  & \text{iff} & a\in v(\pi)_0\\
T\models _v \nextt \psi & \text{iff} & T\models _{v(\pi)^1} \psi\\
T\models _v \psi_1\until\psi_2 & \text{iff} &  \text{there exists} \ i\geq 0 \ \text{such that} \ T\models _{v(\pi)^i} \psi_2, \ \text{and} \\
& & \hspace{1cm}\text{for every} \ 0\leq j <i, \ \text{it holds that} \ T\models _{v(\pi)^j} \psi_1
\end{array}
\]
where $v[\pi\mapsto t]$ denotes the assignment obtained from $v$ by assigning the trace variable $\pi$ to $t$
}



An LTL formula $\f$ over a set $AP$ of atomic propositions can be translated to an NBW $A_\f$ whose language is the set of traces that satisfy $\f$.
The alphabet of $A_\f$ is $2^{AP}$, where each letter marks the set of atomic propositions that are assigned $\true$ in a state along the trace.

Based on this construction, we can translate a hyperLTL formula $\g = \quant_1 x_1 \ldots \quant_k x_k \f$ over $AP$ to an NBH $\A_\g$ over $X = \{x_1,\ldots,x_k\}$, whose quantification condition is $\quant_1 x_1 \ldots \quant_k x_k$. 
The underlying NBW $\hat\A_\g$ is the translation of $\f$ to an NBW. Accordingly, the alphabet of $\hat\A_\g$ is $(2^{AP})^X$.
The NBW $\hat\A_\g$ runs on words that represent traces that are assigned to the $X$ variables, where a letter $\{\sigma_{1_{x_1}},\ldots \sigma_{k_{x_k}}\}$ represents the set of atomic propositions that hold in each of the current states in these traces. That is, for every $i\in[1,k]$, the letter $\sigma_{i_{x_i}}$ is the set of atomic propositions that hold in the current state in the trace that is assigned to $x_i$.
The quantification condition of $\A$, along with the semantics of the quantifiers in $\g$ assure that a hyperword $S$ is accepted by $\A_\g$ iff $S\models\g$. 
Since the translation of an LTL formula to an NBW is exponential in the size of the formula, we have the following. 

\begin{theorem}\label{thrm:hltltonbh}
Every HyperLTL formula $\g = \alpha\f$ can be translated to an NBH $\A_\g$ whose size is exponential in $|\f|$. 
\end{theorem}





==> HyperBuchi.tex <==
\section{Hyperautomata over Infinite Words}\label{sec:hyperbuchi}

We now lift the notion of hyperautomata to infinite words. 
%An infinite word over an alphabet $\Sigma$ is an infinite sequence $\sigma_1\sigma_2\cdots$ of letters from $\Sigma$.
As before, a hyperautomaton $\A$ consists of an underlying automaton which runs on assignments to word variables $\A$. Now, we consider hyperwords that consist of infinite words, 
%({\em hyperinfinite words}, henceforth), 
and accordingly, the underlying automaton runs on assignments of infinite words to the word variables.% We consider a B{\"u}chi acceptance condition.

A {\em nondeterministic B{\"u}chi automaton} (NBW) is a tuple $A 
= \tuple{\Sigma,Q,Q_0,\delta,F}$,
where $\Sigma$, $Q$, $Q_0$, $F$, and $\delta$ are as in Definition~\ref{def:nfa}. 
A run of an NBW $A$ on an infinite word $w=\sigma_1\sigma_2\cdots$ is an infinite sequence of states $r = (q_0,q_1,\ldots)$, such 
that $q_0\in Q_0$, and for every $i>0$, it holds that 
$(q_{i-1},\sigma_i, q_i)\in \delta$.
%
The run is accepting if $r$ visits some state in $F$ infinitely often.
The definitions of acceptance and language are then as for NFA.
%
\stam{
We say that $A$ {\em accepts} $w$ if there exists an accepting run of $A$ on $w$. 
%
The {\em language} of $A$, denoted $\lang{A}$, is the set of all infinite words accepted by $A$. 


\begin{definition}
\label{def:nba}
A {\em nondeterministic B{\"u}chi automaton} (NBW) is a tuple \linebreak $A 
= \tuple{\Sigma,Q,Q_0,\delta,F}$,
where $\Sigma$ is an alphabet, $Q$ is a 
nonempty finite set of {\em states}, $Q_0\subseteq Q$ is a set of {\em initial states}, $F\subseteq Q$ is a set of {\em accepting states}, and 
$\delta\subseteq Q\times\Sigma\times Q$ is a {\em transition relation}.  
\end{definition}
}% of stam
%
We use an NBW as an underlying automaton in a hyperautomaton for hyperwords with infinite words. 

\begin{definition}
A {\em nondeterministic B{\"u}chi hyperword automaton (NBH)} is a hyperautomaton with an underlying NBW. 
\end{definition}

\subsection{Properties of NBH}

%NBWs are closed under the Boolean operations, and their nonemptiness and membership problems are decidable (and are \comp{NL-complete} and \comp{PSPACE-complete}, respectively). 
The results of Section~\ref{sec:nfh_properties} can be lifted to the case of hyperinfinite words, with similar proofs. 
To summarize, we have the following. 

\begin{theorem}
\begin{itemize}
    \item NBH are closed under the Boolean operations.
    \item The nonemptiness problem for NBH$_\exists$ and NBH$_\forall$ is \comp{NL-complete}.
    \item The nonemptiness problem for NBH$_{\exists\forall}$ is \comp{PSPACE-complete}.
    \item The nonemptiness problem for NBH is undecidable.
    \item The $\omega$-regular membership problem for NBH is decidable.
\end{itemize}
\end{theorem}

\input{HLTLtoNBH}

==> biblio.tex <==
\newcommand{\SortNoop}[1]{}
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{ab18}
{\'{A}}brah{\'{a}}m, E., Bonakdarpour, B.: {H}yper{PCTL}: {A} temporal logic
  for probabilistic hyperproperties. In: QEST 2018. pp. 20--35

\bibitem{as85}
Alpern, B., Schneider, F.B.: Defining liveness. Information Processing Letters
  \textbf{21},  181--185 (1985)

\bibitem{bf18}
Bonakdarpour, B., Finkbeiner, B.: The complexity of monitoring hyperproperties.
  In: CSF 2018. pp. 162--174 

\bibitem{bss18}
Bonakdarpour, B., S{\'{a}}nchez, C., Schneider, G.: Monitoring hyperproperties
  by combining static analysis and runtime verification. In: ISoLA 2018. pp. 8--27 

\bibitem{bd02}
Boudol, G., Castellani, I.: Noninterference for concurrent programs and thread
  systems. TCS 2002  \textbf{281}(1-2),  109--130
  

\bibitem{cfkmrs14}
Clarkson, M.R., Finkbeiner, B., Koleini, M., Micinski, K.K., Rabe, M.N.,
  S{\'{a}}nchez, C.: Temporal logics for hyperproperties. In: POST 2014. pp. 265--284
  

\bibitem{cs10}
Clarkson, M.R., Schneider, F.B.: Hyperproperties. Journal of Computer Security
  \textbf{18}(6),  1157--1210 (2010)

\bibitem{cfst19}
Coenen, N., Finkbeiner, B., S{\'{a}}nchez, C., Tentrup, L.: Verifying
  hyperliveness. In: CAV 2019. pp. 121--139

\bibitem{eh86}
Emerson, E.A., Halpern, J.Y.: ``sometimes" and ``not never" revisited: on
  branching versus linear time temporal logic. Journal of the {ACM}
  \textbf{33}(1),  151--178 (1986)

\bibitem{fht19}
Finkbeiner, B., Haas, L., Torfah, H.: Canonical representations of $k$-safety
  hyperproperties. In: CSF 2019. pp. 17--31 

\bibitem{fh16}
Finkbeiner, B., Hahn, C.: Deciding hyperproperties. In: CONCUR 2016. pp. 13:1--13:14

\bibitem{frs15}
Finkbeiner, B., Rabe, M.N., S{\'{a}}nchez, C.: Algorithms for model checking
  {H}yper{LTL} and {H}yper{CTL}*. In: CAV 2015. pp. 30--48 

\bibitem{gm82}
Goguen, J.A., Meseguer, J.: Security policies and security models. In: IEEE
  Symp. on Security and Privacy. pp. 11--20 (1982)

\bibitem{m88}
McCullough, D.: Noninterference and the composability of security properties.
  In: Proceedings of the 1988 {IEEE} Symposium on Security and Privacy. pp.
  177--186 (1988)

\bibitem{p77}
Pnueli, A.: The temporal logic of programs. In: FOCS 1977. pp. 46--57 

\bibitem{ss00}
Sabelfeld, A., Sands, D.: Probabilistic noninterference for multi-threaded
  programs. In: CSFW 2000. pp. 200--214 

\bibitem{vw86}
Vardi, M., Wolper, P.: Automata theoretic techniques for modal logic of
  programs. Journal of Computer and System Sciences  \textbf{32},  183--221
  (1986)

\bibitem{VW94}
Vardi, M., Wolper, P.: Reasoning about infinite computations. Information and
  Computation  \textbf{115}(1),  1--37 (1994)

\bibitem{wzbp19}
Wang, Y., Zarei, M., Bonakdarpour, B., Pajic, M.: Statistical verification of
  hyperproperties for cyber-physical systems. {ACM} Transactions on Embedded
  Computing systems (TECS)  \textbf{18}(5s),  92:1--92:23 (2019)

\bibitem{zm03}
Zdancewic, S., Myers, A.C.: Observational determinism for concurrent program
  security. In: CSFW 2003. p.~29 

\end{thebibliography}

==> bibliography.tex <==
\begin{thebibliography}{10}

\bibitem{ab18}
E.~{\'{A}}brah{\'{a}}m and B.~Bonakdarpour.
\newblock {H}yper{PCTL}: {A} temporal logic for probabilistic hyperproperties.
\newblock In {\em QEST } 2018, p. 20--35.

\bibitem{as85}
B.~Alpern and F.~B. Schneider.
\newblock Defining liveness.
\newblock {\em Information Processing Letters}, 21:181--185, 1985.

\bibitem{bf18}
B.~Bonakdarpour and B.~Finkbeiner.
\newblock The complexity of monitoring hyperproperties.
\newblock In {\em CSF } 2018, p. 162--174.

\bibitem{bss18}
B.~Bonakdarpour, C.~S{\'{a}}nchez, and G.~Schneider.
\newblock Monitoring hyperproperties by combining static analysis and runtime
  verification.
\newblock In {\em ISoLA} 2018, p. 8--27.

\bibitem{bd02}
G.~Boudol and I.~Castellani.
\newblock Noninterference for concurrent programs and thread systems.
\newblock In {\em TCS } 2002, 281(1-2):109--130.

\bibitem{cfkmrs14}
M.~R. Clarkson, B.~Finkbeiner, M.~Koleini, K.~K. Micinski, M.~N. Rabe, and
  C.~S{\'{a}}nchez.
\newblock Temporal logics for hyperproperties.
\newblock In {\em POST} 2014, p. 265--284.

\bibitem{cs10}
M.~R. Clarkson and F.~B. Schneider.
\newblock Hyperproperties.
\newblock {\em Journal of Computer Security}, 18(6):1157--1210, 2010.

\bibitem{cfst19}
N.~Coenen, B.~Finkbeiner, C.~S{\'{a}}nchez, and L.~Tentrup.
\newblock Verifying hyperliveness.
\newblock In {\em CAV } 2019, p. 121--139.

\bibitem{eh86}
E.~A. Emerson and J.~Y. Halpern.
\newblock ``sometimes" and ``not never" revisited: on branching versus linear
  time temporal logic.
\newblock {\em Journal of the {ACM}}, 33(1):151--178, 1986.

\bibitem{fht19}
B.~Finkbeiner, L.~Haas, and H.~Torfah.
\newblock Canonical representations of $k$-safety hyperproperties.
\newblock In {\em CSF } 2019, p. 17--31.

\bibitem{fh16}
B.~Finkbeiner and C.~Hahn.
\newblock Deciding hyperproperties.
\newblock In {\em CONCUR } 2016, p. 13:1--13:14.

\bibitem{frs15}
B.~Finkbeiner, M.~N. Rabe, and C.~S{\'{a}}nchez.
\newblock Algorithms for model checking {H}yper{LTL} and {H}yper{CTL}*.
\newblock In {\em CAV } 2015, p. 30--48.

\bibitem{gm82}
J.~A. Goguen and J.~Meseguer.
\newblock Security policies and security models.
\newblock In {\em IEEE Symp. on Security and Privacy}, p. 11--20, 1982.

\bibitem{m88}
D.~McCullough.
\newblock Noninterference and the composability of security properties.
\newblock In {\em {IEEE} Symposium on Security and Privacy}, 1988, p. 177--186.

\bibitem{p77}
A.~Pnueli.
\newblock The temporal logic of programs.
\newblock In {\em FOCS} 1977, p.  46--57.

\bibitem{ss00}
A.~Sabelfeld and D.~Sands.
\newblock Probabilistic noninterference for multi-threaded programs.
\newblock In {\em CSFW } 2000, p. 200--214.

\bibitem{vw86}
M.Y. Vardi and P.~Wolper.
\newblock Automata theoretic techniques for modal logic of programs.
\newblock {\em Journal of Computer and System Sciences}, 32:183--221, 1986.

\bibitem{VW94}
M.Y. Vardi and P.~Wolper.
\newblock Reasoning about infinite computations.
\newblock {\em Information and Computation}, 115(1):1--37, 1994.

\bibitem{wzbp19}
Y.~Wang, M.~Zarei, B.~Bonakdarpour, and M.~Pajic.
\newblock Statistical verification of hyperproperties for cyber-physical
  systems.
\newblock {\em {ACM} TECS},
  18(5s):92:1--92:23, 2019.

\bibitem{zm03}
S.~Zdancewic and A.~C. Myers.
\newblock Observational determinism for concurrent program security.
\newblock In {\em CSFW } 2003, p.~29.

\end{thebibliography}

==> canonical_forms.tex <==

\subsection{Canonical Forms for the Alternation-Free Fragments}\label{subsec:canonical.forms}

%Throughout this section, we discuss NFH over $\Sigma$ and a set of variables $X$.
We begin with the basic terms on which our canonical forms are based.
\begin{definition}
\begin{enumerate}
\item An $\nfhf$ $\A_\forall$ is {\em sequence complete} if for every word ${\bi w}$, it holds that $\hat{\A_\forall}$ accepts ${\bi w}$ iff it accepts every sequence of ${\bi w}$. 
\item An $\nfhe$ $\A_\exists$ is {\em permutation complete} if for every word 
${\bi w}$, it holds that $\hat \A_\exists$ accepts ${\bi w}$ iff it accepts every permutation of 
${\bi w}$. 
\end{enumerate}
\end{definition}

An $\nfhf$ $\A_\forall$ accepts a hyperword $S$ iff $\hat\A_\forall$ accepts every sequence of size $k$ of $S$. If some sequence is missing from $\lang{\hat\A}$, then removing the rest of the sequences of $S$ from $\lang{\hat\A_\forall}$ does not affect the non-acceptance of $S$. Therefore, the underlying automata of sequence-complete $\nfhf$ only accept necessary sequences. 
Similarly, an $\nfhe$ $\A_\exists$ accepts a hyperword $S$ iff $\hat\A_\exists$ accepts some permutation $p$ of size $k$ of words in $S$. Adding the rest of the permutations of $p$ to $\lang{\hat\A_\exists}$ does not affect the acceptance of $S$. Therefore, the underlying automata of permutation-complete $\nfhe$ only reject the necessary permutations of every hyperword. 
As a conclusion, we have the following.

\begin{lemma}
\label{lem:langeq}
\begin{enumerate}
\item Let $\A_\forall$ be an $\nfhf$, and let $\A'_\forall$ be a sequence-complete $\nfhf$ over $\Sigma$ and $X$ such that for every word ${\bi w}$, the underlying NFA
$\hat{\A'_\forall}$ accepts ${\bi w}$ iff $\hat{\A_\forall}$ accepts every sequence of ${\bi w}$. Then $\hlang{\A_\forall} =\hlang{\A'_\forall}$.
\item Let $\A_\exists$ be an $\nfhe$, and let $\A'_\exists$ be a permutation-complete $\nfhe$ over $\Sigma$ and $X$ such that for every word ${\bi w}$, the underlying NFA $\hat{\A_\exists}$ accepts ${\bi w}$ iff $\hat{\A'_\exists}$ accepts all permutations of ${\bi w}$. 
Then $\hlang{\A_\exists} =\hlang{\A'_\exists}$.
\end{enumerate}

\end{lemma}

Next, we show that we can construct a sequence- or permutation-complete NFH for a given $\nfhf$ or $\nfhe$, respectively. Intuitively, given $\A$,
for every sequence (permutation) $\zeta$ of $(1,\ldots k)$, we construct an NFA that runs on ${\bi w}_\zeta$ in the same way that $\hat\A$ runs on $\bi w$, for every $\bi w$.
The underlying NFA we construct for the $\nfhf$ and $\nfhe$ are the intersection and union, respectively, of all these NFA. 

\begin{lemma}\label{lem:permutation.sequence.complete}
Every $\nfhf$ ($\nfhe$) $\A$ has an equivalent sequence-complete (permutation-complete) $\nfhf$ ($\nfhe$) $\A'$ over the same set of variables. 
\end{lemma}

Finally, as the following theorem shows, sequence- and permutation- complete NFH offer a unified model for the alternation-free fragments.

\begin{theorem}\label{thm:permutation.sequence.complete}
Let $\A_1$ and $\A_2$ be two sequence-complete (permutation-complete) $\nfhf$ ($\nfhe$) over the same set of variables. Then $\hlang{\A_1}=\hlang{\A_2}$ iff  $\lang{\hat\A_1} = \lang{\hat \A_2}$.
\end{theorem}

\stam{
\begin{lemma}
\label{lem:eqseq}
Every $\nfhf$ $\A$ has an equivalent sequence-complete $\nfhf$ $\A'$ over the 
same set of variables. 
\end{lemma}

\begin{lemma}
\label{lem:seqcomp}
Let $\A_1$ and $\A_2$ be two sequence-complete $\nfhf$ over the same set of 
variables $X$.
Then $\lang{\A_1}=\lang{\A_2}$ iff  $\lang{\hat\A_1} = \lang{\hat \A_2}$.
\end{lemma}
}

Regular languages have a canonical form, which are minimal DFA. We use this property to define canonical forms for $\nfhf$ and $\nfhe$ as sequence-complete (permutation-complete) $\nfhf$ ($\nfhe$) with a minimal number of variables and a minimal underlying DFA. 

\stam{

\subsubsection{A Canonical Form for $\nfhe$}

We say that an $\nfhe$ $\A'$ is {\em permutation complete} if for every word 
$w$, it holds that $\hat \A'$ accepts $w$ iff it accepts every permutation of 
$w$. 

\begin{lemma}
\label{lem:premcomp}
Let $\A$ be an $\nfhe$.
Let $\A'$ be a permutation-complete $\nfhe$ over $\Sigma$ and $X$ with the following property: for every word $w$, the underlying NFA $\hat\A$ accepts a word $w$ iff $\hat\A'$ accepts all permutations of $w$. %Notice that this is the dual property of the one listed for $\nfhf$.
Then $\lang{\A} =\lang{\A'}$.
\end{lemma}

\begin{lemma}
\label{lem:eqpermcomp}
Every $\nfhe$ has an equivalent permutation-complete $\nfhe$ over the same set 
of variables. 
\end{lemma}

\begin{lemma}
\label{lem:permcompsame}
Let $\A_1$ and $\A_2$ be two permutation-complete $\nfhe$ over the same set of 
variables $X$.
Then $\lang{\A_1}=\lang{\A_2}$ iff  $\lang{\hat\A_1} = \lang{\hat \A_2}$.
\end{lemma}

We define a canonical form for $\nfhe$ as a minimal deterministic 
permutation-complete $\nfhe$ with a minimal number of variables.


}% of stam








==> canonical_forms_full.tex <==

\subsection{Canonical Forms for Alternation-free Fragment}

Throughout this section, we discuss NFH over an alphabet $\Sigma$ with a set of 
variables $X = \{x_1,x_2,\ldots x_k\}$.

\subsubsection{A Canonical Form for $\nfhf$}

We begin with a canonical form for $\nfhf$. Let $\A$ be an $\nfhf$. 
We say that an $\nfhf$ $\A'$ is {\em sequence complete} if for every word $w$, it holds that $\hat \A'$ accepts $w$ iff it accepts every sequence of $w$. 

\begin{lemma}
\label{lem:langeq}
Let $\A'$ be a sequence complete $\nfhf$ over $\Sigma$ and $X$, such that 
$\hat\A'$ accepts $w$ iff $\hat\A$ accepts every sequence of $w$. 
Then $\lang{\A} =\lang{\A'}$.
\end{lemma}


\begin{lemma}
\label{lem:eqseq}
Every $\nfhf$ $\A$ has an equivalent sequence-complete $\nfhf$ $\A'$ over the 
same set of variables. 
\end{lemma}

\begin{lemma}
\label{lem:seqcomp}
Let $\A_1$ and $\A_2$ be two sequence-complete $\nfhf$ over the same set of 
variables $X$.
Then $\lang{\A_1}=\lang{\A_2}$ iff  $\lang{\hat\A_1} = \lang{\hat \A_2}$.
\end{lemma}

Every NFA has an equivalent DFA, and DFAs have a canonical form, which is a 
minimal DFA. We use this property to define a canonical form for $\nfhf$ as 
minimal deterministic sequence-complete $\nfhf$ with a minimal number of 
variables. 


\subsubsection{A Canonical Form for $\nfhe$}

We say that an $\nfhf$ $\A'$ is {\em permutation complete} if for every word 
$w$, it holds that $\hat \A'$ accepts $w$ iff it accepts every permutation of 
$w$. 

\begin{lemma}
\label{lem:premcomp}
Let $\A$ be an $\nfhe$.
Let $\A'$ be a permutation-complete $\nfhe$ over $\Sigma$ and $X$ with the following property: for every word $w$, the underlying NFA $\hat\A$ accepts a word $w$ iff $\hat\A'$ accepts all permutations of $w$. %Notice that this is the dual property of the one listed for $\nfhf$.
Then $\lang{\A} =\lang{\A'}$.
\end{lemma}

\begin{lemma}
\label{lem:eqpermcomp}
Every $\nfhe$ has an equivalent permutation-complete $\nfhe$ over the same set 
of variables. 
\end{lemma}

\begin{lemma}
\label{lem:permcompsame}
Let $\A_1$ and $\A_2$ be two permutation-complete $\nfhe$ over the same set of 
variables $X$.
Then $\lang{\A_1}=\lang{\A_2}$ iff  $\lang{\hat\A_1} = \lang{\hat \A_2}$.
\end{lemma}

We define a canonical form for $\nfhe$ as a minimal deterministic 
permutation-complete $\nfhe$ with a minimal number of variables.




\stam{

\subsubsection{A canonical form for $\nfhef$}

The canonical form for $\nfhef$ is a combination of the canonical forms for 
$\nfhf$ and $\nfhe$.

We denote an $\nfhef$ $\A$ with a quantification condition $\alpha = \exists 
x_1\ldots \exists x_t\forall k_{t+1}\ldots \forall x_k$ as a $(k,t)-\nfhef$. 

We say that a $(k,t)-\nfhef$ $\A$ is {\em permutation-sequence complete} if 
$\A$ accepts a word $w$ iff $\A$ accepts every sequence $w'$ of $w$ in which 
$(w'[1],\ldots w'[t])$ is a permutation of $(w[1],\ldots w[t])$. 

\begin{lemma}\label{lem:nfhef1}
Let $\A$ be a $(k,t)-\nfhef$. 
Let $\A'$ be a $(k-t)-\nfhef$, with the following property.
$w'\in\lang{\A'}$ iff $w'$ is a sequence of a word $w\in\lang{\hat\A}$ such that
\begin{enumerate}
\item
$(w'[1],\ldots w'[t])$ is a permutation of $(w[1],\ldots w[t])$. 
\item
$w_\zeta\in\lang{\hat\A}$ for every sequence $\zeta$ such that $\zeta = (1,2,\ldots t,i_{t+1},\ldots i_k)$. That is, $\hat\A$ accepts all sequences of $w$ that agree with $w$ on its first $t$ words. 
\end{enumerate}
Then $\lang{\A} = \lang{A'}$.
 \end{lemma}
\begin{proof}
For the first direction, let $S\in\lang{A}$. According to the semantics of the quantifiers, there exist $w_1,\ldots w_t\in S$, such that for every $w_{t+1},\ldots w_{k}$, it holds that $\hat\A$ accepts $\zip(w_1,\ldots w_k)$.
Then, by the semantics of the $\forall$ quantifier, $\hat\A$ accepts all words of the form $\zip(w_1,w_2,\ldots w_t,w'_{t+1},\ldots w'_k)$, where $w'_{t+1},\ldots w'_k$ are taken from $\{w_1,\ldots w_k\}$. Then, by the conditions described above, we have that $\hat\A'$ accepts $\zip(w_1,\ldots w_k)$, and therefore $S\in\lang{A'}$.

For the second direction, let $S\in\lang{A'}$. 
Then there exist $w_1,\ldots w_t\in S$, such that for every $w_{t+1},\ldots w_{k}$, it holds that $\hat\A'$ accepts $w' = \zip(w_1,\ldots w_k)$.
Then, by the conditions described above, $w'$ is a sequence of a word $w\in\lang{A}$ such that $\{w[1],\ldots w[t]\} = \{w'[1], \ldots w'[t]\} = \{w_1,\ldots w_t\}$ (though these words do not necessarily appear in the same order in $w,w'$), and such that $w[i] = w'[i]$ for every $t<i\leq k$. 
Then, by the semantics of the quantifiers, we have that $S\in\lang{\A}$.
\end{proof}

Notice that the $\nfhef$ $\A'$ of Lemma~\ref{lem:nfhef1} is permutation-sequence complete.

\begin{lemma}
Every $(k,t)-\nfhef$ $\A$ has an equivalent permutation-sequence complete $(k,t)-\nfhef$ $\A'$.
\end{lemma}
\begin{proof}
We construct $\A'$ in two steps. 
First, we construct $\A''$ that is the intersection of every $\A_\zeta$ for a sequence $\zeta$ of the form $(1,2,\ldots t, i_{t+1},\ldots i_k)$, as for $\nfhf$ over the last $k-t$ indices, and then we construct $\A'$ as the union of $\A''_\xi$ for every permutation $\xi$ of the form $(i_1,\ldots i_t,t+1,\ldots k)$, as for $\nfhe$ over the first $t$ indices.
\end{proof}

\begin{lemma}
Let $\A_1$ and $\A_2$ be two permutation-sequence complete $(k,t)-\nfhef$.
Then $\lang{\A_1}=\lang{\A_2}$ iff  $\lang{\hat\A_1} = \lang{\hat \A_2}$.
\end{lemma}
\begin{proof}
Suppose that $\lang{\A_1}=\lang{\A_2}$. Let $w\in\lang{\hat\A_1}$. 
Since $\A_1$ is permutation-sequence complete, we have that $w_\zeta\in\lang{\A_1}$ for every sequence $\zeta$ of the form $(1,\ldots t,i_{t+1},\ldots i_k)$. By the semantics of the quantifiers, we have that $\unzip{w}\in\lang{A_1}$.
Therefore, $\unzip{w}\in\lang{A_2}$, and so, according to the semantics of the quantifiers and the order of words in $w$, 
there exists a word $w'\in\lang{\hat\A_2}$ such that $(w'[1],\ldots w'[t])$ is a permutation of $(w[1],\ldots w[t])$, and $(w'[t+1],\ldots w'[k])$ is a permutation of $(w[t+1],\ldots w[k])$. Since $\A_2$ is permutation-sequence complete, we have that $w\in\lang{\hat\A_2}$. A similar argument shows that $\lang{\hat\A_2}\subseteq \lang{\hat\A_1}$.
The second direction is trivial.
\end{proof}

\begin{lemma}
Let $\A$ be a $(k,t)-\nfhef$, such that $k$ is the minimal number of variables needed for expressing $\lang{\A}$.
Then $\hat\A$ accepts a word $w$ in which $w[1],\ldots w[t]$ are all distinct. 
\end{lemma}
\begin{proof}
Suppose by way of contradiction that for every $w\in\lang{\hat\A}$, two of the first $t$ words of in $w$ are equal. Due to the semantics of the $\exists$ quantifier, we can also 
\end{proof}


\begin{lemma}
Let $\A_1$ and $\A_2$ be permutation-sequence complete $\nfhef$ for the same hyperlanguage $\cal L$, both with a minimal set of variables. Then the quantification conditions of $\A_1$ and $\A_2$ are equal.
\end{lemma}
\begin{proof}
Suppose that $\A_1$ is a $(t,k)-\nfhef$, and $\A_2$ is a $(t,m)-\nfhef$.
Suppose by way of contradiction, and without loss of generality, that $t < m$. 
Let $S\in\lang{\A_1}$. 
\end{proof}

We define a canonical form for $\nfhef$ as a minimal deterministic permutation-sequence complete $\nfhef$ with a minimal number of variables. 


}% of stam











==> figures/learning_flow.tex <==
\begin{figure} 

\centering


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\scalebox{.95}{
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,427.3333320617676); %set diagram left start at 0, and has height of 427.3333320617676

%Curve Lines [id:da3242324591734014] 
\draw    (78.05,195.76) .. controls (77.68,166.57) and (91.81,174.17) .. (90.87,193.02) ;
\draw [shift={(90.63,195.76)}, rotate = 276.98] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Rounded Rect [id:dp5230596682902247] 
\draw   (285.46,140.05) .. controls (285.46,135.9) and (288.82,132.53) .. (292.98,132.53) -- (422.81,132.53) .. controls (426.96,132.53) and (430.33,135.9) .. (430.33,140.05) -- (430.33,162.59) .. controls (430.33,166.74) and (426.96,170.11) .. (422.81,170.11) -- (292.98,170.11) .. controls (288.82,170.11) and (285.46,166.74) .. (285.46,162.59) -- cycle ;
%Straight Lines [id:da19996498797143802] 
\draw    (360,195) -- (360,174) ;
\draw [shift={(360,171)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Straight Lines [id:da7742261006504376] 
\draw    (360.15,232.33) -- (360.15,254.42) ;
\draw [shift={(360.15,257.42)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Straight Lines [id:da7240079665223356] 
\draw    (318.59,285.97) -- (147.88,285.97) ;
\draw [shift={(144.88,285.97)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Straight Lines [id:da4355292395155117] 
\draw    (88.79,255.9) -- (88.97,236) ;
\draw [shift={(89,233)}, rotate = 450.53] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Straight Lines [id:da9395518765143251] 
\draw    (140,216) -- (183.56,216) ;
\draw [shift={(186.56,216)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Straight Lines [id:da9876991440040634] 
\draw    (280.98,215.74) -- (316,215.98) ;
\draw [shift={(319,216)}, rotate = 180.4] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Straight Lines [id:da8894863053773812] 
\draw    (318.59,278.87) -- (141.02,231.11) ;
\draw [shift={(138.12,230.33)}, rotate = 375.05] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Rounded Rect [id:dp7304454638728446] 
\draw   (318.59,203.21) .. controls (318.59,199.09) and (321.93,195.76) .. (326.04,195.76) -- (404.26,195.76) .. controls (408.37,195.76) and (411.71,199.09) .. (411.71,203.21) -- (411.71,225.56) .. controls (411.71,229.67) and (408.37,233) .. (404.26,233) -- (326.04,233) .. controls (321.93,233) and (318.59,229.67) .. (318.59,225.56) -- cycle ;
%Straight Lines [id:da989641097303189] 
\draw    (285.46,140.05) -- (142.89,199.6) ;
\draw [shift={(140.12,200.76)}, rotate = 337.33000000000004] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Straight Lines [id:da5782151978812646] 
\draw    (431,147.86) -- (487,147.86) ;
\draw [shift={(490,147.86)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Rounded Rect [id:dp9174543196821443] 
\draw   (186.68,203.21) .. controls (186.68,199.09) and (190.02,195.76) .. (194.13,195.76) -- (272.35,195.76) .. controls (276.46,195.76) and (279.8,199.09) .. (279.8,203.21) -- (279.8,225.56) .. controls (279.8,229.67) and (276.46,233) .. (272.35,233) -- (194.13,233) .. controls (190.02,233) and (186.68,229.67) .. (186.68,225.56) -- cycle ;
%Rounded Rect [id:dp013423076978946291] 
\draw   (318.59,263.62) .. controls (318.59,259.51) and (321.93,256.17) .. (326.04,256.17) -- (404.26,256.17) .. controls (408.37,256.17) and (411.71,259.51) .. (411.71,263.62) -- (411.71,285.97) .. controls (411.71,290.08) and (408.37,293.42) .. (404.26,293.42) -- (326.04,293.42) .. controls (321.93,293.42) and (318.59,290.08) .. (318.59,285.97) -- cycle ;
%Rounded Rect [id:dp7630850927481354] 
\draw   (47.01,203.54) .. controls (47.01,199.42) and (50.35,196.09) .. (54.46,196.09) -- (132.68,196.09) .. controls (136.79,196.09) and (140.12,199.42) .. (140.12,203.54) -- (140.12,225.89) .. controls (140.12,230) and (136.79,233.33) .. (132.68,233.33) -- (54.46,233.33) .. controls (50.35,233.33) and (47.01,230) .. (47.01,225.89) -- cycle ;
%Rounded Rect [id:dp6612685395327704] 
\draw   (50,263.2) .. controls (50,259.09) and (53.34,255.76) .. (57.45,255.76) -- (135.67,255.76) .. controls (139.78,255.76) and (143.11,259.09) .. (143.11,263.2) -- (143.11,285.55) .. controls (143.11,289.66) and (139.78,293) .. (135.67,293) -- (57.45,293) .. controls (53.34,293) and (50,289.66) .. (50,285.55) -- cycle ;
%Straight Lines [id:da6707127407283302] 
\draw    (29.79,211.24) -- (43.84,211.24) ;
\draw [shift={(46.84,211.24)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;


% Text Node
\draw (141.81,182.12) node   [align=left] {$ $};
% Text Node
\draw (93.57,214.71) node   [align=left] {$\displaystyle T${\fontfamily{ptm}\selectfont  }~closed \\and consistent?};
% Text Node
\draw (98.22,162.32) node   [align=left] {no: membership queries};
% Text Node
\draw (233.24,214.38) node   [align=left] {construct $\displaystyle \mathcal{A}$};
% Text Node
\draw (357.89,151.32) node   [align=left] {permutation/sequence \\complete?};
% Text Node
\draw (229.13,150.68) node  [rotate=-337.24] [align=left] {no: add cex~{\fontfamily{ptm}\selectfont  }$\displaystyle w$};
% Text Node
\draw (365.15,214.38) node   [align=left] {equivalent?};
% Text Node
\draw (394.44,242.91) node  [rotate=-359.45] [align=left] {no: cex $\displaystyle S$};
% Text Node
\draw (365.15,274.8) node  [rotate=-359.45] [align=left] {$\displaystyle |S| >k?$};
% Text Node
\draw (378.6,183.41) node  [rotate=-359.45] [align=left] {yes};
% Text Node
\draw (163.6,207.37) node  [rotate=-359.45] [align=left] {yes};
% Text Node
\draw (291.5,204) node   [align=left] {{\fontfamily{ptm}\selectfont  }$\displaystyle \mathcal{A}$};
% Text Node
\draw (269.92,254.66) node  [rotate=-14.77] [align=left] {no: add cex $\displaystyle S${\fontfamily{ptm}\selectfont  }};
% Text Node
\draw (237.84,277.89) node  [rotate=-359.61] [align=left] {yes};
% Text Node
\draw (458.14,137.71) node  [rotate=-359.45] [align=left] {yes: {\fontfamily{ptm}\selectfont  }$\displaystyle \mathcal{A}$};
% Text Node
\draw (115.57,245.15) node  [rotate=-359.61] [align=left] {add~{\fontfamily{ptm}\selectfont  }$\displaystyle S${\fontfamily{ptm}\selectfont  }};
% Text Node
\draw (96.56,274.38) node   [align=left] {{\fontfamily{ptm}\selectfont  }$\displaystyle T\leftarrow \uparrow ^{k'}_{k}( T)${\fontfamily{ptm}\selectfont  }};


\end{tikzpicture}
}

\caption{The learning process flow for $\nfhf$ and $\nfhe$.}
\label{fig:learning_flow}
\vspace{-3mm}
\end{figure}


==> hyperautomata.tex <==
\subsection{Hyperautomata}
\label{sec:ha}

%\subsection{The General Idea}




We now turn to formally define  hyperautomata.
%of both types. 

\input{NFH}
%\input{NBH}



==> proofs.tex <==
\section{Proofs}

We present several terms and notations which we use throughout the following proofs.
%
Recall that we represent an assignment $v:X\rightarrow S$ as a word assignment $\wass{w}{v}$.
Conversely, a word ${\bi w}$ over $(\Sigma\cup\{\#\})^X$ represents an assignment $\assw{v}{w}:X\rightarrow \Sigma^*$, where $\assw{v}{w}(x_i)$ is formed by concatenating the letters of $\Sigma$ that are assigned to $x_i$ in the letters of ${\bi w}$
%For example the word ${\bi w} = \{a_{x_1},b_{x_2}\}\{b_{x_1},\#_{x_2}\}$ represents the assignment $x_1\mapsto ab, x_2\mapsto b$. 
We denote the set of all such words $\{\assw{v}{w}(x_1),\ldots,\assw{v}{w}(x_k)\}$ by $S({\bi w})$.
Since we only allow padding at the end of a word, if a padding occurs in the middle of $\bi w$, then $\bi w$ does not represent a legal assignment. Notice that this occurs iff ${\bi w}$ contains two consecutive letters ${\bi w}_i{\bi w}_{i+1}$ such that ${\bi w}_i(x) = \#$ and ${\bi w}_{i+1}(x)\neq \#$ for some $x\in X$.  
We call ${\bi w}$ {\em legal} if $\assw{v}{w}$ represents a legal assignment from $X$ to $\Sigma^*$.

Consider a function $g:A\rightarrow B$ where $A,B$ are some sets. 
The {\em range} of $g$, denoted $\range(g)$ is the set $\{g(a)| a\in A\}$.

A {\em sequence} of $g$ is a function $g':A\rightarrow B$ such that $\range(g')\subseteq \range(g)$. 
A {\em permutation} of $g$ is a function $g':A\rightarrow B$ such that $\range(g') = \range(g)$.
We extend the notions of sequences and permutations to word assignments. Let ${\bi w}$ be a word over $\hat\Sigma$. A sequence of ${\bi w}$ is a word ${\bi w'}$ such that $S(w')\subseteq S(w)$, and a permutation of ${\bi w}$ is a word ${\bi w'}$ such that $S(w')=S(w)$.


\subsection*{Theorem~\ref{thm:nfh.operations}}

\begin{proof}
{\bf Complementation. }
Let $\A$ be an NFH. The NFA $\hat \A$ 
can be complemented with respect to its language over $\hat\Sigma$ to an NFA 
$\overline{\hat{\A}}$. 
Then for every assignment $v:X\rightarrow S$, it holds that $\hat \A$ accepts 
$\wass{w}{v}$ iff $\overline{\hat{\A}}$ does not accept $\wass{w}{v}$.
%
Let $\overline{\alpha}$ be the quantification condition obtained from $\alpha$ 
by replacing every $\exists$ with $\forall$ and vice versa. 
We can prove by induction on $\alpha$ that $\overline{\A}$, the NFH 
whose 
underlying NFA is $\overline{\hat{\A}}$, and whose quantification 
condition is 
$\overline{\alpha}$, accepts $\overline {\hlang{\A}}$.
%
The size of $\overline{\A}$ is exponential in $|Q|$, due to the complementation construction for $\hat\A$.

Now, let $\A_1 = 
\tuple{\Sigma,X,Q,Q_0,\delta_1,F_1,\alpha_1}$ and $\A_2= 
\tuple{\Sigma,Y,P,P_0,\delta_2,F_2,\alpha_2}$ be two NFH with $|X|=k$ and 
$|Y|=k'$ variables, respectively.




\bigbreak
\noindent{\bf Union.}
We construct an NFH 
$\A_{\cup} = \tuple{\Sigma,X\cup Y, Q\cup P\cup\{p_1,p_2\},  Q_0\cup P_0, \delta, 
F_1\cup F_2\cup\{p_1,p_2\}, \alpha}$, where $\alpha = \alpha_1\alpha_2$ (that is, we concatenate the two quantification conditions), and where $\delta$ is defined as follows. 
\begin{itemize}
\item For every $(q_1\xrightarrow{f} q_2)\in 
\delta_1$ we set $(q_1\xrightarrow{f\cup g} q_2)\in \delta$ for every $g\in (\Sigma\cup\{\#\})^{Y}$. 

\item
For every $(q_1\xrightarrow{f} q_2)\in \delta_2$ we set $(q_1\xrightarrow{f\cup g} q_2)\in \delta$ for every $g\in (\Sigma\cup\{\#\})^{X}$. 

\item
For every $q\in F_1$, we set 
$(q\xrightarrow{\{\#\}^X\cup g}p_1),(p_1\xrightarrow{\{\#\}^X\cup g}p_1)\in \delta$
for every $g\in (\Sigma\cup\{\#\})^{Y}$.

\item
For every $q\in F_2$, we set $(q\xrightarrow{g\cup\{\#\}^{Y}}p_2),(p_2\xrightarrow{g\cup\{\#\}^{Y}}p_2)\in \delta$ for every $g\in (\Sigma\cup\{\#\})^{X}$.

%\item Dual transitions for every $(q_1\xrightarrow{f} q_2)\in \delta_2$ and every $q\in F_2$.
\end{itemize}

Let $S$ be a hyperword. 
For every $v:(X\cup Y)\rightarrow S$, it holds that if $\wass{w}{v|_X}\in\lang{\hat\A_1}$, then $\wass{w}{v}\in\lang{\hat\A_{\cup}}$. Indeed, according to our construction, every word assigned to the $Y$ variables is accepted in the $\A_1$ component of the construction, and so it satisfies both types of quantifiers.
A similar argument holds for $v|_Y$ and $\A_2$.

Also, according to our construction, for every $v:(X\cup Y)\rightarrow S$,  if $\wass{w}{v}\in\lang{\hat\A_{\cup}}$, then either $\wass{w}{v|_X}\in\lang{\hat\A_1}$, or $\wass{w}{v|_Y}\in\lang{\hat\A_2}$. 
%
As a conclusion, we have that $\hlang{\A_{\cup}} = \hlang{\A_1}\cup\hlang{\A_2}$. 

The state space of $\A_\cup$ is linear in the state spaces of $\A_1,\A_2$. 
However, the size of the alphabet of $\A_\cup$ may be exponentially larger than 
that of $\A_1$ and $\A_2$, since we augment each letter with all functions from $Y$ to $\Sigma\cup\{\#\}$ (in $\A_1$) and from $X$ to $\Sigma\cup\{\#\}$ (in $\A_2$).

\bigbreak
\noindent{\bf Intersection.}
The proof follows the closure of regular hyperlanguages under union and complementation. However, we also offer a direct translation, which avoids the need to complement. 
We construct an NFH 
$\A_\cap = \tuple{\Sigma,X\cup Y, (Q\cup \{q\}) \times (P\cup \{p\}), (Q_0\times P_0), \delta, 
(F_1\cup\{q\}) \times (F_2\cup\{p\}), \alpha_1\alpha_2}$, where $\delta$ is defined as follows. 
\begin{itemize}
    \item For every $(q_1\xrightarrow {f} q_2)\in 
\delta_1$ and every $(p_1\xrightarrow {g} p_2)\in\delta_2$, we have 
%
$$\Big((q_1,p_1)\xrightarrow{f\cup g} (q_2,p_2)\Big)\in\delta$$
%
\item For every $q_1\in F_1, (p_1 \xrightarrow{g} p_2)\in \delta_2$ we have
%
$$\Big((q_1,p_1)\xrightarrow {\{\#\}^X \cup g}(q,p_2)\Big), \Big((q,p_1)\xrightarrow {\{\#\}^k\cup g}(q,p_2)\Big) \in \delta$$
%

%\item Dual transitions for every $(q_1\xrightarrow {f} q_2)\in \delta_1$ and $p_1\in F_2$.
%, we have
%

\item
For every $(q_1\xrightarrow {f} q_2)\in \delta_1$ and $p_1\in F_2$, we have
$$\Big((q_1,p_1)\xrightarrow{f\cup\{\#\}^Y}(q_2,p)\Big), \Big((q_1,p)\xrightarrow{f\cup\{\#\}^Y}(q_2,p)\Big)\in \delta$$

\end{itemize}
%
Intuitively, the role of $q,p$ is to keep reading $\{\#\}^X$ and $\{\#\}^Y$ after 
the word read by $\hat\A_1$ or $\hat\A_2$, respectively, has ended. 

The NFH $\hat{\A_\cap}$ simultaneously reads two word assignments 
%\zip(w_1, w_2, \ldots, w_k)$ and $\zip(w'_1,w'_2,\ldots w'_{k'})$ 
that are read along $\hat\A_1$ and 
$\hat\A_2$, 
respectively, and accepts iff both word assignments are accepted. The correctness 
follows from the fact that for $v:(X\cup Y)\rightarrow S$, we have that 
$\wass{w}{v}$ is accepted by $\hat\A$ iff $\wass{w}{v|_X}$ and $\wass{w}{v|_Y}$ are 
accepted by $\hat\A_1$ and $\hat\A_2$, respectively. 
This construction is polynomial in the sizes of $\A_1$ and $\A_2$.


\stam{
Complementing $\A$ amounts to dualizing its quantification condition (replacing every $\exists$ with $\forall$ and vice versa), and complementing $\hat\A$ via the standard construction for NFA.

Now, let $\A_1$ and $\A_2$ be two NFH over $\Sigma$, with the variables $X$ and $Y$, respectively.
The NFH $\A_{\cap}$ for $\hlang{\A_1}\cap \hlang{\A_2}$ is based on the product construction of $\hat\A_1$ and $\hat\A_2$.
The quantification condition of $\A_{\cap}$ is $\alpha_1 \cdot \alpha_2$. 
The underlying automaton $\hat\A_{\cap}$ advances simultaneously on both $\A_1$ 
and $\A_2$: when $\hat\A_1$ and $\hat\A_2$ run on word assignments ${\bi w_1}$ 
and ${\bi w_2}$, respectively, 
$\hat\A_{\cap}$ runs on a word assignment ${\bi w_1}\cup{\bi w_2}$, which represents both assignments ${\bi w_1}$ and ${\bi w_2}$, and accepts only if both 
$\hat\A_1$ and $\hat\A_2$ accept.
To run on both assignments simultaneously, every letter in $\A_{\cap}$ is of the type $f_1\cup f_2$, where $f_1:X\rightarrow (\Sigma\cup\{\#\})$ is a letter in $\hat\Sigma_1$, and $f_2:Y\rightarrow (\Sigma\cup\{\#\})$ is a letter in $\hat\Sigma_2$.

Similarly, the NFH $\A_{\cup}$ for $\hlang{\A_1}\cup \hlang{\A_2}$ is based on the union construction of $\hat\A_1$ and $\hat\A_2$.
The quantification condition of $\A_{\cup}$ is again $\alpha_1\cdot \alpha_2$. 
The underlying automaton $\hat\A_{\cup}$ advances either on $\A_1$ or $\A_2$. For every word word assignemt $\bi w$ read by $\hat\A_1$, the NFH $\hat\A_{\cup}$ reads ${\bi w}\cup{\bi w'}$, for every ${\bi w}'\in \hat\Sigma_2^*$, and dually, for every word $\bi w$ read by $\hat\A_2$, the NFH $\hat\A_{\cup}$ reads ${\bi w'}\cup{\bi w}$, for every ${\bi w}'\in \hat\Sigma_1^*$.
}% of stam
\end{proof}

% undecidability, nonempitness of nfhe,nfhf


\subsection*{Theorem~\ref{thm:nonemptiness}}

\begin{proof}

{\bf $\nfhe$ and $\nfhf$.}
The lower bound for both fragments follows from the \comp{NL-hardness} of the nonemptiness problem for NFA. 

We turn to the upper bound, and begin with $\nfhe$. Let $\A_\exists$ be an $\nfhe$. 
We claim that $\A_\exists$ is nonempty iff $\hat\A_\exists$ accepts some legal 
word ${\bi w}$. The first direction is trivial. For the second direction, let 
${\bi w}\in\lang{\hat\A_\exists}$. By 
assigning $v(x_i) = \assw{v}{w}(x_i)$ for every $x_i\in X$, we get $\wass{w}{v} = {\bi w}$, and 
according to the semantics of $\exists$, we have that $\A_\exists$ accepts $S({\bi w})$. 
To check whether $\hat\A_\exists$ accepts a legal word, we can run a 
reachability check on-the-fly, while advancing from a letter $\sigma$ to the 
next letter $\sigma'$ only if $\sigma'$ assigns $\#$ to all variables for which $\sigma$ assigns $\#$. 
While each transition $T = q\xrightarrow{f} p$ in 
$\hat\A$ is of size $k$, we can encode $T$ as 
 a set of size $k$ of encodings of 
transitions of type $q \xrightarrow {(x_i,\sigma_i)} p$ with a binary encoding of 
$p,q,\sigma_i$, as well as $i,t$, where $t$ marks the index of $T$ within the 
set of transitions of $\hat\A$. 
Therefore, the reachability test can be performed within space that is logarithmic in the size of $\A_\exists$.

Now, let $\A_\forall$ be an $\nfhf$ over $X$. We claim that $\A_\forall$ is 
nonempty iff $\A_\forall$ accepts a hyperword of size $1$. 
For the first direction, let $S\in\hlang{\A_\forall}$. Then, by the semantics of 
$\forall$, we have that for every assignment $v:X\rightarrow S$, it holds that 
$\wass{w}{v}\in\lang{\hat{\A_\forall}}$. Let $u\in S$, and let $v_u(x_i) = u$ for every 
$x_i\in X$. Then, in particular, $\wass{w}{v_u}\in\lang{\hat{\A_\forall}}$. Then for every assignment $v:X\rightarrow \{u\}$ (which consists of the 
single assignment $v_u$), it holds that $\hat{\A_\forall}$ accepts $\wass{w}{v}$, 
and therefore $\A_\forall$ accepts $\{u\}$. 
The second direction is trivial. 

To check whether $\A_\forall$ accepts a hyperword of size $1$, we restrict the reachability test on $\hat\A_\forall$ to  
letters over $\hat\Sigma$ that represent fixed functions. 

\bigbreak
{\bf $\nfhef$. }
We prove a \comp{PSPACE} upper bound.
Let $m$ be the number of $\exists$ quantifiers in $\alpha$, and 
let $S\in\hlang{\A}$. Then, according to the semantics of the quantifiers, 
there exist $w_1,\ldots w_m \in S$, such that for every assignment 
$v:X\rightarrow S$ in which $v(x_i) = w_i$ for every $1\leq i\leq m$, it holds that $\hat\A$ accepts $\wass{w}{v}$. Let $v:X\rightarrow S$ be such an 
assignment. Then, $\hat\A$ accepts 
$\wass{w}{v'}$ for every sequence $v'$ of $v$ that agrees with $v$ on its assignments to $x_1,\ldots,x_m$, and in particular, for such sequences whose range is $\{w_1,\ldots,w_m\}$. 
Therefore, by the semantics of the quantifiers, we have that $\{w_1,\ldots,w_m\}$ is 
in $\hlang{\A}$. The second direction is trivial.

We call $\wass{w}{v'}$ as described above a {\em witness to the nonemptiness of 
$\A$}.
%, i.e., $\wass{w}{v_\zeta}$ is an instantiation of the existential quantifiers.
%
We construct an NFA $A$ based on $\hat\A$ that is nonempty iff $\hat\A$ accepts 
a witness to the nonemptiness of $\A$.

Let $\Gamma$ be the set of all functions of the type $\zeta:[1,k]\rightarrow [1,m]$ such that $\zeta(i)=i$ for every $i\in[1,m]$, and such that $\range(\zeta) = [1,m]$.
For a letter assignment $f = \{\sigma_{1_{x_1}},\ldots \sigma_{k_{x_k}}\}$, we denote by $f_\zeta$ the letter assignment $\{\sigma_{\zeta(1)_{x_1}},\ldots, \sigma_{\zeta(k)_{x_k}}\}$. 

For every function $\zeta\in\Gamma$, we construct 
an NFA $A_\zeta = \tuple{ \hat\Sigma,Q,Q_0,\delta_\zeta,F}$, where for every 
$q\xrightarrow{g} q'$ in $\delta$, 
we have $q\xrightarrow{f} q'$ in 
$\delta_\zeta$, for every $f$ that occurs in $\hat\A$ for which $f_\zeta = g$.
Intuitively, for every run of $A_{\zeta}$ on a word ${\bi w}$ there exists a similar run of $\hat\A$ on the sequence of ${\bi w}$ that matches $\zeta$. Therefore, $\hat\A$ accepts a witness ${\bi w}$ to the nonemptiness of $\A$ iff ${\bi w}\in\lang{A_\zeta}$ for every $\zeta\in\Gamma$. 

We define $A = \bigcap_{\zeta\in\Gamma} A_\zeta$.
Then $\hat\A$ accepts a witness to the nonemptiness of $\A$ iff $A$ is 
nonempty. 

Since $|\Gamma| = m^{k-m}$, the state space of $A$ is of size $O(n^{m^{k-m}})$, where $n=|Q|$, 
and its alphabet is of size $|\hat\Sigma|$. 
%
Notice that for $\A$ to be nonempty, $\delta$ must be of size at least 
$|(\Sigma\cup {\#})|^{(k-m)}$, to account for all the sequences of letters in 
the words assigned to the variables under $\forall$ quantifiers (otherwise, we 
can immediately return ``empty''). Therefore, $|\hat\A|$ is $O(n\cdot 
|\Sigma|^k)$. 
We then have that the size of $A$ is $O(|\hat \A|^k)$.  
%
If the number $k-m$ of $\forall$ quantifiers is fixed, then $m^{k-m}$ is 
polynomial in $k$. However, now $|\hat\A|$ may be polynomial in $n,k$, and $|\Sigma|$, 
and so in this case as well, the size of $A$ is $O(|\hat A|^k)$. 

Since the nonemptiness problem for NFA is \comp{NL-complete}, the problem for $\nfhef$ 
can be decided in space of size that is polynomial in $|{\hat\A}|$. 


\bigbreak
{\bf General NFH.}
We mimic the proof idea in~\cite{fh16}, which uses a reduction from the {\em 
Post correspondence problem (PCP)}, which is known to be undecidable.
%
A PCP instance is a collection $C$ of dominoes of the form:
$$ \Bigg\{\Big[\frac{u_1}{v_1} \Big], 
\Big[\frac{u_2}{v_2} \Big],\dots, \Big[\frac{u_k}{v_k} \Big] \Bigg\}$$
where for all $i \in [1, k]$, we have $v_i,u_i \in 
\{a,b\}^*$.
%\alphabet_{\mathit{pcp}}^*$.
%
The problem is to decide whether there exists a finite sequence of the dominoes 
of the form
%
$$\Big[\frac{u_{i_1}}{v_{i_1}} \Big]\Big[\frac{u_{i_2}}{v_{i_2}} \Big] \cdots 
\Big[\frac{u_{i_m}}{v_{i_m}} \Big]$$
%
where each index $i_j \in [1, k]$, such that the upper and lower finite 
strings of the dominoes are equal, i.e.,
%
$$ u_{i_1}u_{i_2}\cdots{}u_{i_m} = v_{i_1}v_{i_2}\cdots{}v_{i_m}$$
%
For example, if the set of dominoes is
%
$$ C_{\mathsf{exmp}} = \Bigg\{ \Big[\frac{ab}{b}\Big], 
\Big[\frac{ba}{a}\Big],\Big[\frac{a}{aba}\Big] \Bigg\} $$
%
Then, a possible solution is the following sequence of dominoes from 
$C_{\mathsf{exmp}}$: 
%
$$\mathsf{sol} = \Big[\frac{a}{aba}\Big]\Big[\frac{ba}{a}\Big] 
\Big[\frac{ab}{b}\Big ].  $$

%

Given an instance $C$ of PCP, we encode a solution as a word $w_{sol}$ over the 
following alphabet:
%
$$\alphabet = \Big\{\frac{\sigma}{\sigma'} \mid \sigma,\sigma'\in\{a,b,{\dot 
a},{\dot b}, \$\}\Big\}.$$
%
Intuitively, $\dot{\sigma}$ marks the beginning of a new domino, and 
$\$$ marks the end of a sequence of the upper or lower parts of the dominoes 
sequence.

%For a word $w = \frac{\sigma_1}{\sigma'_1}   \frac{\sigma_2}{\sigma'_2}  
% \cdots  \frac{\sigma_n}{\sigma'_n} \in \Sigma^* $, we call $\sigma_1\cdots 
% \sigma_n$ the {\em upper part} of $w$, and the word $\sigma'_1\cdots 
%\sigma'_n$ the {\em lower part} of $w$. 

We note that $w_{sol}$ encodes a legal solution iff the following conditions are 
met:

\begin{enumerate}
    \item For every $ \frac{\sigma}{\sigma'}  $ that occurs in $w_{sol}$, it 
holds that $\sigma,\sigma'$ represent the same domino letter (both $a$ or both 
$b$, either dotted or undotted).
    \item The number of dotted letters in the upper part of $w_{sol}$ is equal 
to the number of dotted letters in the lower part of $w_{sol}$.
    \item $w_{sol}$ starts with two dotted letters, and the word $u_i$ between 
the $i$'th and $i+1$'th dotted letters in the upper part of $w_{sol}$, and the 
word $v_i$ between the corresponding dotted letters in the lower part of 
$w_{sol}$ are such that $ [\frac{u_i}{v_i}]  \in C$, for every $i$.
\end{enumerate}

We call a word that represents the removal of the first $k$ dominoes from 
$w_{sol}$ 
a {\em partial solution}, denoted by $w_{sol,k}$.
Note that the upper and lower parts of $w_{sol,k}$ are not necessarily of equal 
lengths (in terms of $a$ and $b$ sequences), since the upper and lower parts of 
a domino may be of different lengths, and so we use letter $\$$ to pad 
the end of the encoding in the shorter of the two parts. 

We construct an NFH $\A$, which, intuitively, expresses the following ideas: 
$(1)$ There exists an encoding $w_{sol}$ of a solution to $C$, and $(2)$ For 
every $w_{sol,k}\neq \epsilon$ in a hyperword $S$ accepted by $\A$, the word 
$w_{sol,k+1}$ is also in $S$. 

$\hlang{\A}$ is then the set of all hyperwords that contain an encoded solution 
$w_{sol}$, as well as all its suffixes obtained by removing a prefix of dominoes 
from $w_{sol}$. This ensures that $w_{sol}$ indeed encodes a legal solution. For example, a matching hyperword $S$ (for the solution 
$\mathsf{sol}$ discussed earlier) that is accepted by $\A$ is:
%
$$ S = \{  w_{sol} = \frac{\dot a}{\dot a}   \frac{\dot b}{b}   \frac{a}{a}   
\frac{\dot a}{\dot a}   \frac{b}{\dot b} ,
w_{sol,1} = \frac{\dot b}{\dot a}\frac{a}{\dot b}\frac{\dot a}{\$}\frac{b}{\$}, 
w_{sol,2} = \frac{\dot a}{\dot b}\frac{b}{\$}, w_{sol,3} = \epsilon
\} $$

Thus, the quantification condition of $\A$ is $\alpha = \forall x_1\exists x_2 
\exists x_3$, where $x_1$ is to be assigned a potential partial solution 
$w_{sol,k}$, and $x_2$ is to be assigned $w_{sol,k+1}$, and $x_3$ is to be 
assigned $w_{sol}$.  

During a run on a hyperword $S$ and an assignment $v:\{x_1,x_2,x_3\}\rightarrow 
S$, the NFH $\A$ checks that the upper and lower letters of $w_{sol}$ all match.
In addition, $\A$ checks that the first domino of $v(x_1)$ is indeed in $C$, and 
that $v(x_2)$ is obtained from $v(x_1)$ by removing the first tile. 
$\A$ performs the latter task by checking that the upper and lower parts of 
$v(x_2)$ are the upper and lower parts of $v(x_1)$ that have been ``shifted'' 
back appropriately. That is, if the first tile in $v(x_2)$ is the encoding of 
$[\frac{w_i}{v_i}]$, then $\A$ uses states to remember, at each point, the last 
$|w_i|$ letters of the upper part of $v(x_2)$ and the last $|v_i|$ letters of 
the lower part of $v(x_2)$, and verifies, at each point, that the next letter in 
$v(x_1)$ matches the matching letter remembered by the state.
\end{proof}
























\stam{

\subsection*{Theorem~\ref{thm:nfh.operations}}
\begin{proof}
{\bf Complementation. }
Let $\A$ be an NFH. The NFA $\hat \A$ 
can be complemented with respect to its language over $\hat\Sigma$ to an NFA 
$\overline{\hat{\A}}$. 
Then for every assignment $v:X\rightarrow S$, it holds that $\hat \A$ accepts 
$\wass{w}{v}$ iff $\overline{\hat{\A}}$ does not accept $\wass{w}{v}$.
%
Let $\overline{\alpha}$ be the quantification condition obtained from $\alpha$ 
by replacing every $\exists$ with $\forall$ and vice versa. 
We can prove by induction on $\alpha$ that $\overline{\A}$, the NFH 
whose 
underlying NFA is $\overline{\hat{\A}}$, and whose quantification 
condition is 
$\overline{\alpha}$, accepts $\overline {\hlang{\A}}$.
%
The size of $\overline{\A}$ is exponential in $|Q|$, due to the complementation construction for $\hat\A$.

Now, let $\A_1 = 
\tuple{\Sigma,X,Q,Q_0,\delta_1,F_1,\alpha_1}$ and $\A_2= 
\tuple{\Sigma,Y,P,P_0,\delta_2,F_2,\alpha_2}$ be two NFH with $|X|=k$ and 
$|Y|=k'$ variables, respectively.


\bigbreak
\noindent{\bf Union.}
We construct an NFH 
$\A_{\cup} = \tuple{\Sigma,X\cup Y, Q\cup P\cup\{p_1,p_2\},  Q_0\cup P_0, \delta, 
F_1\cup F_2\cup\{p_1,p_2\}, \alpha}$, where $\alpha = \alpha_1\alpha_2$ (that is, we concatenate the two quantification conditions), and where $\delta$ is defined as follows. 

\begin{itemize}

\item For every $(q_1\xrightarrow{f} q_2)\in 
\delta_1$ we set $(q_1\xrightarrow{f\cup g} q_2)\in \delta$ for every $g\in (\Sigma\cup\{\#\})^{Y}$. 


\item
For every $(q_1\xrightarrow{f} q_2)\in 
\delta_2$ we set $(q_1\xrightarrow{f\cup g} q_2)\in 
\delta$ for every $g\in (\Sigma\cup\{\#\})^{X}$. 

\item
For every $q\in F_1$, we set 
$(q\xrightarrow{\{\#\}^X\cup g}p_1),(p_1\xrightarrow{\{\#\}^X\cup g}p_1)\in \delta$
for every $g\in (\Sigma\cup\{\#\})^{Y}$.

\item
For every $q\in F_2$, we set 
$(q\xrightarrow{g\cup\{\#\}^{Y}}p_2),(p_2\xrightarrow{g\cup\{\#\}^{Y}}p_2)\in \delta$
for every $g\in (\Sigma\cup\{\#\})^{X}$.
\end{itemize}

Let $S$ be a hyperword. 
For every $v:(X\cup Y)\rightarrow S$, it holds that if $\wass{w}{v|_X}\in\lang{\hat\A_1}$, then $\wass{w}{v}\in\lang{\hat\A_{\cup}}$. Indeed, according to our construction, every word assigned to the $Y$ variables is accepted in the $\A_1$ component of the construction, and so it satisfies both types of quantifiers.
A similar argument holds for $v|_Y$ and $\A_2$.

Also, according to our construction, for every $v:(X\cup Y)\rightarrow S$,  if $\wass{w}{v}\in\lang{\hat\A_{\cup}}$, then either $\wass{w}{v|_X}\in\lang{\hat\A_1}$, or $\wass{w}{v|_Y}\in\lang{\hat\A_2}$. 
%
As a conclusion, we have that $\hlang{\A_{\cup}} = \hlang{\A_1}\cup\hlang{\A_2}$. 

The state space of $\A_\cup$ is linear in the state spaces of $\A_1,\A_2$. 
However, the size of the alphabet of $\A_\cup$ may be exponentially larger than 
that of $\A_1$ and $\A_2$, since we augment each letter with all functions from $Y$ to $\Sigma\cup\{\#\}$ (in $\A_1$) and from $X$ to $\Sigma\cup\{\#\}$ (in $\A_2$).

\bigbreak
\noindent{\bf Intersection.}
The proof follows the closure under union and complementation. However, we
also offer a direct translation, which avoids the need to complement. 
We construct an NFH 
$\A_\cap = \tuple{\Sigma,X\cup Y, (Q\cup \{q\}) \times (P\cup \{p\}), (Q_0\times P_0), \delta, 
(F_1\cup\{q\}) \times (F_2\cup\{p\}), \alpha_1\alpha_2}$, where $\delta$ is defined as follows. 
\begin{itemize}
    \item For every $(q_1\xrightarrow {f} q_2)\in 
\delta_1$ and every $(p_1\xrightarrow {g} p_2)\in\delta_2$, we have 
%
$\Big((q_1,p_1)\xrightarrow{f\cup g} (q_2,p_2)\Big)\in\delta$
%
\item For every $q_1\in F_1, (p_1 \xrightarrow{g} p_2)\in \delta_2$ we have
%
$$\Big((q_1,p_1)\xrightarrow {\{\#\}^X \cup g}(q,p_2)\Big), \Big((q,p_1)\xrightarrow {\{\#\}^k\cup g}(q,p_2)\Big) \in \delta$$
%
\item For every $(q_1\xrightarrow {f} q_2)\in 
\delta_1$ and $p_1\in F_2$, we have
%
$$\Big((q_1,p_1)\xrightarrow 
{f\cup\{\#\}^Y}(q_2,p)\Big), \Big((q_1,p)\xrightarrow 
{f\cup\{\#\}^Y}(q_2,p)\Big)\in \delta$$
\end{itemize}
%
Intuitively, the role of $q,p$ is to keep reading $\{\#\}^X$ and $\{\#\}^Y$ after 
the word read by $\hat\A_1$ or $\hat\A_2$, respectively, has ended. 

The NFH $\hat{\A_\cap}$ simultaneously reads two word assignments 
%\zip(w_1, w_2, \ldots, w_k)$ and $\zip(w'_1,w'_2,\ldots w'_{k'})$ 
that are read along $\hat\A_1$ and 
$\hat\A_2$, 
respectively, and accepts iff both word assignments are accepted. The correctness 
follows from the fact that for $v:(X\cup Y)\rightarrow S$, we have that 
$\wass{w}{v}$ is accepted by $\hat\A$ iff $\wass{w}{v|_X}$ and $\wass{w}{v|_Y}$ are 
accepted by $\hat\A_1$ and $\hat\A_2$, respectively. 

This construction is polynomial in the sizes of $\A_1$ and $\A_2$.
\end{proof}






\subsection*{Theorem~\ref{thm:nfhef.nonemptiness}}

\begin{proof}
We begin with the upper bound.
Let $S\in\hlang{\A}$. Then, according to the semantics of the quantifiers, 
there exist $w_1,\ldots w_m \in S$, such that for every assignment 
$v:X\rightarrow S$ in which $v(x_i) = w_i$ for every $1\leq i\leq m$, it holds that $\hat\A$ accepts $\wass{w}{v}$. Let $v:X\rightarrow S$ be such an 
assignment. Then, $\hat\A$ accepts 
$\wass{w}{v'}$ for every sequence $v'$ of $v$ that agrees with $v$ on its assignments to $x_1,\ldots,x_m$, and in particular, for such sequences whose range is $\{w_1,\ldots,w_m\}$. 
Therefore, by the semantics of the quantifiers, we have that $\{w_1,\ldots,w_m\}$ is 
in $\hlang{\A}$. The second direction is trivial.

We call $\wass{w}{v'}$ as described above a {\em witness to the nonemptiness of 
$\A$}.
%, i.e., $\wass{w}{v_\zeta}$ is an instantiation of the existential quantifiers.
%
We construct an NFA $A$ based on $\hat\A$ that is nonempty iff $\hat\A$ accepts 
a witness to the nonemptiness of $\A$.

Let $\Gamma$ be the set of all functions of the type $\zeta:[1,k]\rightarrow [1,m]$ such that $\zeta(i)=i$ for every $i\in[1,m]$, and such that $\range(\zeta) = [1,m]$.
For a letter assignment $f = \{\sigma_{1_{x_1}},\ldots \sigma_{k_{x_k}}\}$, we denote by $f_\zeta$ the letter assignment $\{\sigma_{\zeta(1)_{x_1}},\ldots, \sigma_{\zeta_{k_{x_k}}}\}$. 

For every function $\zeta\in\Gamma$, we construct 
an NFA $A_\zeta = \tuple{ \hat\Sigma,Q,Q_0,\delta_\zeta,F}$, where for every 
$q\xrightarrow{g} q'$ in $\delta$, 
we have $q\xrightarrow{f} q'$ in 
$\delta_\zeta$, for every $f$ that occurs in $\hat\A$ for which $f_\zeta = g$.
Intuitively, for every run of $A_{\zeta}$ on a word ${\bi w}$ there exists a similar of $\hat\A$ on the sequence of ${\bi w}$ that matches $\zeta$. Therefore, $\hat\A$ accepts a witness ${\bi w}$ to the nonemptiness of $\A$ iff ${\bi w}\in\lang{A_\zeta}$ for every $\zeta\in\Gamma$. 

We define $A = \bigcap_{\zeta\in\Gamma} A_\zeta$.
Then $\hat\A$ accepts a witness to the nonemptiness of $\A$ iff $A$ is 
nonempty. 

Since $|\Gamma| = m^{k-m}$, the state space of $A$ is of size $O(n^{m^{k-m}})$, where $n=|Q|$, 
and its alphabet is of size $|\hat\Sigma|$. 
%
Notice that for $\A$ to be nonempty, $\delta$ must be of size at least 
$|(\Sigma\cup {\#})|^{(k-m)}$, to account for all the sequences of letters in 
the words assigned to the variables under $\forall$ quantifiers (otherwise, we 
can immediately return ``empty''). Therefore, $|\hat\A|$ is $O(n\cdot 
|\Sigma|^k)$. 
We then have that the size of $A$ is $O(|\hat \A|^k)$.  
%
If the number $k-m$ of $\forall$ quantifiers is fixed, then $m^{k-m}$ is 
polynomial in $k$. However, now $|\hat\A|$ may be polynomial in $n,k$, and $|\Sigma|$, 
and so in this case as well, the size of $A$ is $O(|\hat A|^k)$. 

Since the nonemptiness problem for NFA is \comp{NL-complete}, the problem for $\nfhef$ 
can be decided in space of size that is polynomial in $|{\hat\A}|$. 

\bigbreak
\noindent{\bf \comp{PSPACE hardness}}
For the lower bound, we show a reduction from a polynomial version of the {\em corridor tiling problem}, %~\cite{Boas97}, defined as follows.
We are given a finite set $T$ of tiles, two relations $V \subseteq T \times T$ 
and $H \subseteq T \times T$,
an initial tile $t_0$, a final tile $t_f$, and a bound $n>0$.
We have to decide whether there is some $m>0$ and a tiling of a $n \times m$-grid such that
(1) The tile $t_0$ is in the bottom left corner and the tile $t_f$ is in the top 
right corner,
(2) A horizontal condition: every pair of horizontal neighbors is in $H$, and
(3) A vertical condition: every pair of vertical neighbors is in $V$.
%
When $n$ is given in unary notation, the problem is known to be 
\comp{PSPACE-complete}.
Given an instance $C$ of the tiling problem, we construct an $\nfhef$ $\A$ that is nonempty iff $C$ has a solution. 
We encode a solution to $C$ as a word $w_{sol} =w_1\cdot w_2\cdot w_m\$$ over 
$\Sigma = T\cup\{1,2,\ldots n,\$\}$, where the word $w_i$, of the form $1\cdot t_{1,i}\cdot 2 \cdot t_{2,i},\ldots n\cdot 
t_{n,i}$, describes the contents of row $i$. 

To check that $w_{sol}$ indeed encodes a solution, we need to make sure that:
\begin{enumerate}
\item $w_1$ begins with $t_0$ and $w_m$ ends with $t_f\$$.
\item $w_i$ is of the correct form.
\item Within every $w_i$, it holds that $(t_{j,i},t_{j+1,i})\in H$.
\item For $w_i,w_{i+1}$, it holds that $(t_{j,i}, t_{j,i+1})\in V$ for every $j\in[1,n]$.
\end{enumerate} 

Verifying items $1-3$ is easy via an NFA of size $O(n|H|)$.  
The main obstacle is item $4$. 

We describe an $\nfhef$ $\A = \tuple{T\cup \{0,1,2,\ldots n,\$\}, 
\{y_1,y_2,y_3,x_1,\ldots x_{\log(n)}\}, Q, \{q_0\},\delta, F, \alpha}$ that is 
nonempty iff there exists a word that satisfies items $1-4$.
The quantification condition $\alpha$ is $\exists y_1\exists y_2 \exists y_3\forall 
x_1 \ldots \forall x_{\log(n)}$.
The NFH $\A$ only proceeds on letters whose assignments to $y_1,y_1,y_3$ is $r,0,1$, respectively, where $r\in T\cup\{1,\ldots n,\$\}$. Notice that this means that $\A$
requires the existence of the words $0^{|w_{sol}|}$ and $1^{|w_{sol}|}$ (the $0$ word and $1$ word, henceforth).
$\A$ makes sure that the word assigned to $y_1$ matches a correct solution 
w.r.t. items $1-3$ described above.  
We proceed to describe how to handle the requirement for $V$. 
We need to make sure that for every position $j$ in a row, the tile in position $j$ in the next row matches the current one w.r.t. $V$. We can use a state $q_j$ to remember the tile in position $j$, and compare it to the tile in the next occurrence of $j$. The problem is avoiding having to check all positions 
simultaneously, which would require exponentially many states. To this end, we use $\log(n)$ copies of the $0$ and $1$ words to form a binary encoding of the position $j$ that is to be remembered. The $\log(n)$ $\forall$ conditions make sure that every position within $1-n$ is checked.  

We limit the checks to words in which $x_1,\ldots x_{\log(n)}$ are the $0$ or $1$ words, by having $\hat\A$ accept every word in which there is a letter that is not over $0,1$ that is assigned to the $x$ variables. This takes care of accepting all cases in which the word assigned to $y_1$ is also assigned to one of the $x$ variables. 

To check that $x_1,\ldots x_{\log(n)}$ are the $0$ or $1$ words, $\hat\A$ checks 
that the letter assignments to these variables remain constant throughout the run. 
In these cases, upon reading the first letter, $\hat\A$ remembers the value $j$ that is encoded by the constant assignments to $x_1,\ldots x_{\log(n)}$ in a state, and makes sure that throughout the run, the tile that occurs in the assignment to $y_1$ in position $j$ in the current row matches the tile in position $j$ in the next row. 

We construct a similar reduction for the case that the number of $\forall$ 
quantifiers is fixed: instead of encoding the position by $\log(n)$ bits, we can 
directly specify the position by a word of the form $j^*$, for every $j\in[1,n]$. 
Accordingly, we construct an $\nfhef$ over $\{x, y_1,\ldots y_{n},z\}$, with a 
quantification condition $\alpha = \exists x\exists y_1 \ldots \exists 
y_{n}\forall z$. The NFA $\hat\A$ advances only on letters whose assignments to 
$y_1,\ldots y_n$ are always $1,2,\ldots n$, respectively, and checks only words assigned to $z$ that are some constant $1\leq j\leq n$. Notice that the fixed assignments to the $y$ variables leads to $\delta$ of polynomial size.  
In a hyperword accepted by $\A$, the word assigned to $x$ is $w_{sol}$, and the word assigned to $z$ specifies which index should be checked for conforming to $V$.
\end{proof}


\subsection*{Theorem~\ref{thm:nfh.membership.finite}}

\begin{proof}
We can decide the membership of $S$ in $\hlang{\A}$ by iterating over all relevant assignments from $X$ to $S$, and for every such assignment $v$, checking on-the-fly whether $\wass{w}{v}$ is accepted by $\hat\A$. 
This algorithm uses space of size that is polynomial in $k$ and logarithmic in $|\A|$ and in $|S|$. 

In the case that $k' = O(\log k)$, an \comp{NP} upper bound is met by iterating over all assignments to the variables under $\forall$, while guessing assignments to the variables under $\exists$. For every such assignment $v$, checking whether $\wass{w}{v}\in\lang{\hat\A}$ can be done on-the-fly. 

We show \comp{NP-hardness} for this case by a reduction from the Hamiltonian cycle problem. 
Given a graph $G = \tuple{V,E}$ where $V = \{v_1,v_2,\ldots, v_n\}$ and 
$|E|=m$, we construct an $\nfhe$ $\A$ over $\{0,1\}$ with $n$ states, $n$ variables, $\delta$ of size $m$, and a hyperword $S$ of size $n$, as follows. $S = \{w_1,\ldots, w_n\}$, where $w_i$ is the word over $\{0,1\}$ in which all letters are $0$ except for the $i$'th. 
The structure of $\hat\A$ is identical to that of $G$, and we set $Q_0 = F = \{v_1\}$. For the transition relation, for every $(v_i,v_j)\in E$, we have $(v_i, f_i,v_j)\in \delta$, where $\f_i$ assigns $0$ to all variables except for $x_i$. 
Intuitively, the $i$'th letter in an accepting run of $\hat\A$ marks traversing 
$v_i$. Assigning $w_j$ to $x_i$ means that the $j$'th step of the run 
traverses $v_i$. Since the words in $w$ make sure that every $v\in V$ is 
traversed exactly once, and that the run on them is of length $n$, we have that $\A$ accepts $S$ iff there exists some ordering of the words in $S$ that matches a Hamiltonian cycle in $G$.

\noindent{\it remark}
To account for all the assignments to the $\forall$ variables, $\delta$ -- and therefore, $\hat\A$ -- must be of size at least $2^{k'}$ (otherwise, we can return ``no'').
We then have that if $k = O(k')$, then space of size $k$ is logarithmic in $|\hat\A|$, and so the problem in this case can be solved within logarithmic space.
A matching NL lower bound follows from the membership problem for NFA. 
\end{proof}


\subsection*{Theorem~\ref{thrm:membershipFULL}}

\begin{proof}
Let $A = \tuple{\Sigma, P, P_0, \rho,F}$ be an NFA, and let $\A = \tuple{\Sigma, 
\{x_1,\ldots, x_k\}, Q, Q_0, \delta, {\cal F},\alpha}$ be an NFH. 

First, we construct an NFA $A'=\tuple{\Sigma\cup\{\#\}, P', P'_0, \rho', F'}$
by extending the alphabet of $A$ to $\Sigma\cup\{\#\}$, adding a new and 
accepting state $p_f$ to $P$ with a self-loop labeled by $\#$, and transitions 
labeled by $\#$ from every $q\in F$ to $p_f$. 
The language of $A'$ is then $\lang{A}\cdot \#^*$.  
We describe a recursive procedure (iterating over $\alpha$) for deciding 
whether $\lang{A}\in\hlang{\A}$.

For the case that $k=1$, it is easy to see that if $\alpha = \exists x_1$, then 
$\lang{A}\in\hlang{\A}$ iff $\lang{A}\cap \lang{\hat{\A}} \neq \emptyset$.
Otherwise, if $\alpha = \forall x_1$, then $\lang{A}\in\hlang{\A}$ iff 
$\lang{A}\notin \hlang{\overline{\A}}$, where $\overline{\A}$ is the NFH for $\overline{\hlang{\A}}$ described in Theorem~\ref{thm:nfh.operations}. 
Notice that the quantification condition for $\overline{\A}$
is $\exists x_1$, and so this conforms to the base case.

For $k>1$, we construct a sequence of NFH $\A_1, \A_2, \ldots, \A_k$. 
If $\quant_1 = \exists$ then we set $\A_1 = \A$, and otherwise we set $\A_1 = \overline{\A}$.
Let $\A_i = \tuple{\Sigma, \{x_i,\ldots, x_k\}, Q_i, 
Q^0_i, \delta_i, {\cal F}_i,\alpha_i}$.
If $\alpha_i$ starts with $\exists$, then 
we construct $\A_{i+1}$ as follows. 

The set of variables of $\A_{i+1}$ is $\{x_{i+1},\ldots, x_k\}$, and the 
quantification condition $\alpha_{i+1}$ is \linebreak $\quant_{i+1}x_{i+1}\cdots 
\quant_kx_k$, for $\alpha_i = \quant_ix_i \quant_{i+1}\cdots \quant_kx_k$. 
The set of states of $\A_{i+1}$ is $ Q_i\times P'$, and the set of initial 
states is $Q_i^0\times P_0$. The set of accepting states is ${\cal F}_i\times 
F'$.
For every 
$(q\xrightarrow{f}q')\in\delta_i$ and every 
$(p\xrightarrow{f(x_i)}p')\in \rho$, we have 
$((q,p)\xrightarrow{f\setminus{\sigma_{i_{x_i}}}}(q',p'))\in\delta_{i+1}$. 
Then, $\hat\A_{i+1}$ accepts a word assignment $\wass{w}{v}$ iff there 
exists a word $u\in \lang{A}$, such that $\hat\A_{i}$ accepts 
$\wass{w}{v\setminus\{x_1\mapsto u\}}$. 

 Let $v:\{x_{i},\ldots, x_k\}\rightarrow \lang{A}$.
Then $\lang{A}\models _v (\alpha_i,\A_i)$ iff there exists $w\in \lang{A}$ such that $\lang{A}\models_{v[x_i\mapsto w]} (\alpha_{i+1},\A_i)$.
For an assignment $v':\{x_{i+1},\ldots, x_k\}\rightarrow \lang{A}$, it holds 
that 
$\wass{w}{v'}$ is accepted by $\hat{\A}_{i+1}$ iff there exists a word $w\in \lang{A}$ such that $\wass{w}{v'}\in\lang{\hat{\A}_i}$, where $v = v'\cup \{x_i\mapsto w\}$. 
Therefore, we have that $\lang{A}\models_{v[x_i\rightarrow 
w]}(\alpha_{i},\A_i)$ 
iff $\lang{A}\models_{v'} (\alpha_{i+1}, \A_{i+1})$, that is, 
$\lang{A}\in\hlang{\A_i}$ iff $\lang{A}\in\hlang{\A_{i+1}}$. 

If $\alpha_i$ starts with $\forall$, then we have that $\lang{A}\in \hlang{\A_i}$ iff 
$\lang{A}\notin \overline{\hlang{\A_i}}$. We construct $\overline{\A_{i}}$ for 
$\overline{\hlang{\A_i}}$ as described in Theorem~\ref{thm:nfh.operations}. The 
quantification condition of $\overline{\A_{i}}$ then begins with $\exists x_i$, and we apply the previous case, and construct $\A_{i+1}$ w.r.t. $\overline{\A_{i}}$, to check for non-membership.

Every $\forall$ quantifier requires complementation, which is exponential in $n$, the number of states in $\A$. Therefore, in the worst case, the complexity of this algorithm is $O(2^{2^{...^{|Q||A|}}})$, where the tower is of height $k$. If the number of $\forall$ quantifiers is fixed, then the complexity is $O(|Q||A|^k)$. 
\end{proof}


\subsection*{Theorem~\ref{thrm:containment}}

\begin{proof}
For the lower bound, we show a reduction from the containment problem for NFA, which is known to be \comp{PSPACE-hard}.
Let $A_1,A_2$ be NFA. We ``convert'' them to NFH $\A_1,\A_2$ by adding to both a single variable $x$ and a quantification condition $\forall x$, and replacing every $\sigma\in \Sigma$ with $\sigma_x$.
By the semantics of the $\forall$ quantifier, we have that $\hlang{\A_1} = \{S | S\subseteq \lang{A_1}\}$, and similarly for $\A_2$. 
Therefore, we have that $\hlang{\A_1}\subseteq \hlang{\A_2}$ iff $\lang{A_1}\subseteq \lang{A_2}$.

For the upper bound, first notice that complementing an $\nfhf$ yields an $\nfhe$, and vice versa. 
Consider two NFH $\A_1$ and $\A_2$.
%, where $\A_1,\A_2\in\nfhf,\nfhe$. 
Then $\hlang{\A_1}\subseteq\hlang{\A_2}$ iff 
$\hlang{\A_1}\cap\overline{\hlang{\A_2}}  =  \emptyset$. 
We can use the constructions in the proof of Theorem~\ref{thm:nfh.operations} 
to compute a matching NFH $\A = 
\A_1\cap\overline{\A_2}$, and check its nonemptiness.
The complementation construction is exponential in $n_2$, the number of states 
of $\A_2$, and the intersection construction is polynomial in $|\A_1|, 
|\overline{\A_2}|$. 

If $\A_1\in\nfhe$ and $\A_2\in\nfhf$ or vice versa, then $\A$ is an $\nfhe$ or $\nfhf$, respectively, whose nonemptiness can be decided in space that is logarithmic in $|\A|$. 

Now, consider the case where $\A_1$ and $\A_2$ are both $\nfhe$ or both $\nfhf$.
It follows from the proof of Theorem~\ref{thm:nfh.operations}, that for two NFH $\A,\A'$, the quantification condition of $\A\cap\A'$ may be any 
interleaving of the quantification conditions of $\A$ and $\A'$. Therefore, if $\A_1,\A_2\in\nfhe$ or $\A_1,\A_2\in\nfhf$, we can construct $\A$ to be an $\nfhef$. 
This is also the case when $\A_1\in\nfhef$ and $\A_2\in\nfhe$ or $\A_2\in\nfhf$.

Either $\A_2$ or $\overline{\A_2}$ is an $\nfhf$, whose underlying NFA has a transition relation of size that is exponential in $k$ (otherwise the $\nfhf$ is empty). The same holds for $\A_1\in\nfhef$. The PSPACE upper bound of Theorem~\ref{thm:nfhef.nonemptiness} is derived from the number of variables and not from the state-space of the NFH. Therefore, while $|\bar{\A_2}|$ is exponential in the number of states of $\A_2$, checking the nonemptiness of $\A$ is in \comp{PSPACE}. 
\end{proof}

}%of stam

\iffalse

\subsection*{Theorem~\ref{thrm:hltltonbh}}
\begin{proof}

%\subsection{Alternating B{\"u}chi Automata}

To describe the construction, we first define {\em Alternating B{\"u}chi Automata} (ABW) \cite{DBLP:conf/litp/MullerS84}. 
We begin with some preliminary terms.

Given a finite set $D$, a \emph{$D$-tree} is a set $T\subseteq D^*$ such that $T$ is prefix-closed. A {\em node} of $T$ is a word in $T$, and the {\em root} of $T$ is the empty word $\epsilon$. 
A {\em path} to a node $u=d_1 d_2\cdots d_n$ in $T$ is the sequence of prefixes $\epsilon, d_1, d_1d_2,\ldots ,d_1d_2\cdots d_n$ of $u$.
A {\em successor} of a node $u \in T$ is of the form $u \cdot d$ where $d\in D$.
For $i\geq 0$, the $i$'th {\em level} in $T$ is the set of words of length $i$ in $T$. 

Given a set $L$, an \emph{$L$-labeled $D$-tree} is a pair $\langle T,f\rangle$ where $T$ is a $D$-tree, and $f:T\rightarrow L$ is a labeling function that labels each node in $T$ by an element of $L$. 

An ABW is a tuple $\B=\langle\Sigma, Q, q_0, \delta, F\rangle$ where $\Sigma, Q, q_0$ and $F$ are as in NBW. The transition relation is $\delta: Q\times \Sigma \rightarrow {B^+}(Q)$, where ${B^+}(Q)$ is the set of positive Boolean formulas over the set of states as well as $\{\mathit{true, false} \}$. That is, formulas that include only the Boolean operators $\wedge$ and $\vee$\footnote{In particular, the negation operator is not included.}. For example, if $\delta(q, a) = (q_1 \wedge q_2) \vee q_3$, then, by reading $a$ from $q$, the ABW $\B$ moves either to both $q_1$ and $q_2$, or to $q_3$. %We assume that $\delta$ is given in disjunctive normal form (DNF). 

A \emph{run} of $\B$ on a word $w=w_1w_2\ldots$ is a $Q$-labeled $Q$-tree, in which the $i$'th level corresponds to the set of states that $\B$ reaches after reading $w_i$.
The root is labeled by $q_0$. For every $q$-labeled node $u$ in level $i$, the set of labels of the children of $u$ is a minimal set (with repect to inclusion) that satisfies $\delta(q,w_i)$. For example, if $\delta(q, a) = (q_1 \wedge q_2) \vee q_3$, and $w_i=a$, and $u$ is a $q$-labeled node on level $i-~1$, then $u$ has either two children labeled $q_1$ and $q_2$, or a single child labeled $q_3$. 
Hence, disjunctions in the transitions are equivalent to non-deterministic choices and influence the number of different run trees on a word, and conjunctions induce a split to two or more successors within the run tree. 
A run is \emph{accepting} if every infinite path in the run tree visits a state from $F$ infinitely often, and every finite path ends with $\true$. That is, the last node on the path is on some level $n$ and is labeled by $q$ such that $\true$ satisfies $\delta(q,w_n)$.
The notions of acceptance and language are as in NBWs.

Every ABW can be translated to an NBW with an exponential blow-up.

We proceed to describe the translation of a hyperLTL formula to NBH. 
Let $\g = \quant_1 x_1 \ldots \quant_k x_k \f$ be a hyperLTL formula. over a set  $AP$ of atomic propositions.
We construct an ABW $\A_\g$ over $(2^{AP})^k$ that accepts a hyperword $S$ iff $S\models\f$. Our construction is directly based on Vardi and Wolper's construction for ABW from LTL. 
The set of states $S$ is $sub(\f)$, the set of sub-formulas of $\f$, the initial state is $\f$, the set of accepting states are all subformulas of the type $\neg \f_1\until\f_2$.
To define the transition relation $\delta$, 
we first define the {\em dual} formula $\overline{\alpha}$ for a formula $\alpha$, as follows. Let $\alpha_1,\alpha_2$ be formulas over $S$. 
\begin{itemize}
    \item $\overline{\true} = \false$ and $\overline{\false}=\true$.
    \item $\overline{\alpha} = \neg\overline{\alpha}$, for $\alpha\in S$.
    \item $\overline{\alpha_1\wedge\alpha_2} = \overline{\alpha_1}\vee\overline{\alpha_2}$.
    \item $\overline{\alpha_1\vee \alpha_2} = \overline{\alpha_1}\wedge\overline{\alpha_2}$.
    \item

\end{itemize}

The transition relation $\delta$ is as follows. 
\begin{itemize}
\item $\delta(a_{x_i},\sigma) = \true$ if $a\in\sigma[i]$, and $\false$ otherwise. 
\item $\delta(\nextt \f_1, \sigma) =  \f_1$.
\item $\delta(\f_1\vee \f_2,\sigma) = \delta(\f_1,\sigma)\vee \delta(\f_2,\sigma)$.
\item $\delta(\neg \f_1) = \overline{\delta(\f_1)}$.
\item $\delta(\f_1 \until \f_2, \sigma) = \delta(\f_2,\sigma)\vee (\delta(\f_1,\sigma) \wedge (\f_1\until\f_2))$. 
\end{itemize}

Finally, the quantification condition of $\A_\g$ is $\quant_1 x_1 \ldots \quant_k x_k$. 
\end{proof}

\fi

==> regular_membership_proof.tex <==
Let $A = \tuple{\Sigma, P, P_0, \rho,F}$ be an NFA with $n$ states.

We first extend the alphabet of $A$ to $\Sigma\cup\{\#\}$, and extend its language to $\lang{A}\cdot\{\#\}^*$.
We next describe a procedure for deciding whether $\lang{A}\in\hlang{\A}$.

For the case that $k=1$, if $\alpha = \exists x_1$, then 
$\lang{A}\in\hlang{\A}$ iff $\lang{A}\cap \lang{\hat{\A}} \neq \emptyset$.
Otherwise, if $\alpha = \forall x_1$, then $\lang{A}\in\hlang{\A}$ iff 
$\lang{A}\notin \hlang{\overline{\A}}$, where $\overline{\A}$ is the NFH for $\overline{\hlang{\A}}$. 
The quantification condition for $\overline{\A}$
is $\exists x_1$, conforming to the base case.

For $k>1$, we construct a sequence of NFA $A_k,A_{k-1} \ldots, A_1$ as follows.
Initially,  $A_{k} = \hat\A$.
Let $A_i = \tuple{\Sigma_i, Q_i, 
Q^0_i, \delta_i, {\cal F}_i}$.
If $\quant_i = \exists$ , then 
we construct $A_{i-1}$ as follows. 
The set of states of $A_{i-1}$ is $Q_i\times P$, and the set of initial 
states is $Q_i^0\times P_0$. The set of accepting states is ${\cal F}_i\times F$.
For every 
$(q\xrightarrow{f}q')\in\delta_i$ and every 
$(p\xrightarrow{f(x_i)}p')\in \rho$, we have 
$((q,p)\xrightarrow{f\setminus{\{\sigma_{i_{x_i}}}\}}(q',p'))\in\delta_{i-1}$. We denote this construction by $A\cap_{x_i} A_i$.
Then, $A_{i-1}$ accepts a word assignment $\wass{w}{v}$ iff there 
exists a word $u\in \lang{A}$, such that $A_{i}$ accepts 
$\wass{w}{v\cup\{x_i\mapsto u\}}$. 

If $\quant_i = \forall$, then  we set $A_{i-1} = \overline{A\cap_{x_i} \overline{A_i}}$
Notice that $A_{i-1}$ accepts a word assignment $\wass{w}{v}$ iff for every $u\in \lang{A}$, it holds that $A_{i}$ accepts 
$\wass{w}{v\cup\{x_i\mapsto u\}}$. 

For $i\in [1,k]$, let $\A_{i}$ be the NFH whose quantification condition is $\alpha_{i} = \quant_1 x_1\cdots \quant_{i} x_{i}$, and whose underlying NFA is $A_i$. Then, according to the construction of $A_{i-1}$, we have that $\lang{A}\in\hlang{\A_i}$ iff $\lang{A}\in\hlang{\A_{i-1}}$. 

The NFH $\A_1$ has a single variable, and we can now apply the base case.

Every $\forall$ quantifier requires complementation, which is exponential in $n$.
Therefore, in the worst case, the complexity of this algorithm is $O(2^{2^{...^{|Q||A|}}})$, where the tower is of height $k$. If the number of $\forall$ quantifiers is fixed, then the complexity is $O(|Q||A|^k)$. 
